Multi-Wavelength, Optical (VI) and Near-Infrared (JHK) Calibration of the Tip of the Red Giant Branch Method based on Milky Way Globular Clusters

Using high precision ground-based photometry for 46 low-reddening Galactic globular clusters, in conjunction with Gaia DR2 proper motions for member star selection, we have calibrated the zero point of the tip of the red giant branch (TRGB) method at two optical ($VI$) and three near-infrared ($JHK$) wavelengths. In doing so, we utilized the sharply-defined zero-age horizontal branch (ZAHB) of these clusters to relatively calibrate our cluster sample into a composite color-magnitude diagram spanning a wide range of metallicities, before setting the absolute zero point of this composite using the geometric detached eclipsing binary distance to the cluster $\omega$ Centauri. The $I-$band zero point we measure [$M_I = -4.056 \pm 0.02 \text{ (stat}) \pm 0.10 \text{ (sys)} $] agrees to within one sigma of the two previously published independent calibrations, using TRGB stars in the LMC [$M_I = $ -4.047 mag; Freedman et al. 2019, 2020] and in the maser galaxy NGC 4258 [$M_{F814W} = $ -4.051 mag; Jang et al. 2020]. We also find close agreement for our $J,H,K$ zero points to several literature studies.

==> table3.tex <==
\begin{deluxetable}{l c c c }
\tablecolumns{4}
% \tablewidth{0pt}
% \tabletypesize{\footnotesize}
\tabletypesize{\small}
\tablecaption{\label{tab:NIR_results}
NIR TRGB Slopes and Zeropoints}
\tablehead{
\colhead{Filter} & \colhead{Slope} & \colhead{$M^{I}_{\rm TRGB}$}  & \colhead{Note}}
\startdata
1 & -0.99 $\pm $xx (stat) & c & c \\
2 & -0.99  $\pm $xx (stat) & c & c \\
3& -0.99 $\pm $xx (stat) & c & c \\
\hline
\enddata
\vspace{-3em}
\tablecaption{Caption goes here.}
\end{deluxetable}
